Deep Multi-Task Learning for Joint Localization, Perception, and Prediction

Over the last few years, we have witnessed tremendous progress on many subtasks of autonomous driving, including perception, motion forecasting, and motion planning. However, these systems often assume that the car is accurately localized against a high-definition map. In this paper we question this assumption, and investigate the issues that arise in state-of-the-art autonomy stacks under localization error. Based on our observations, we design a system that jointly performs perception, prediction, and localization. Our architecture is able to reuse computation between both tasks, and is thus able to correct localization errors efficiently. We show experiments on a large-scale autonomy dataset, demonstrating the efficiency and accuracy of our proposed approach.

==> sections/__latexindent_temp.tex <==

\begin{figure*}[t]
	\centering
	% Raw diagram @ https://drive.google.com/file/d/1iVoqrveqas88b5f_Q2LWKyT0L8efTsfv/view?usp=sharing
	\includegraphics[width=0.95\linewidth,trim=10mm 125mm 102mm 10mm,clip=true]{imgs/LPnP_diagram.pdf}
	\caption{The architecture of the combined localization and perception model.}
	\label{fig:architecture}
\end{figure*}

\section{Joint Localization, Perception, \& Prediction}
\label{sec:method}

We now formulate a model that performs joint localization and PnP (LPnP).
First, we explain the key challenges that we would like our system to overcome,
and then explain our design choices in detail.

% \subsection{Key challenges}

\paragraph{Latency:}
In order to provide a safe ride,
a self-driving car must react quickly to changes in its environment.
In practice, this means that we must minimize the time form perception to action.
In a na{\"i}ve, cascaded autonomy system, the latency of each component adds up linearly,
which may result in unacceptable latency.

To reduce the latency of the localization system,
it is common to use Bayesian filtering to provide high-frequency pose updates.
In this case, a belief about the pose is maintained over time and updated through the
continuous integration of different levels of evidence from wheel autoencoders, IMUs, or camera and LiDAR sensing.
In this context, the external sensing step
(\eg carried out via iterative closest point alignment between the LiDAR reading and an HD map)
typically carries the strongest evidence, but is also the most expensive part of the system.
Therefore, it is critical to keep the latency of the sensing step of the localization filter low.

\paragraph{Learning-based localization:}
Localization systems with learned components are typically better
at discerning semantic aspects of the scene that are traditionally
hard to discriminate with purely geometric features
(\eg growing vegetation, tree stumps, and dynamic objects),
and have the potential of being more invariant to appearance changes due to 
season, weather, and illumination~\cite{pit30m}.
Therefore, we would like to incorporate a learning-based localization component on our system.
Moreover, since PnP systems are typically heavily driven by learning,
it should be possible to incorporate learning-based localization with
by sharing computation between the two modules, resulting in
reduced overhead to the overall LPnP system.

\paragraph{Training and deployment:}
% We would like the joint LPnP system to incur overall a smaller technical debt than a classical autonomy stack.
% Following the terminology of Sculley~\etal~\cite{sculley2015debt},
% we argue that developing and serving a single model inherently reducess the process management debt
% (\ie the debt associated with handling multiple models),
% but may incur additional 
We would like our joint LPnP system to be easier to train and deploy than its classical counterpart.
Given the large amounts of ML infrastructure invested around PnP systems
(\eg on dataset curation, labelling, active learning, and monitoring),
it makes sense to design a localization subsystem that can be trained as a smaller addition
to a larger PnP model.
This should also make it easier to iterate on lightweight localization modules
without the need to retraind the more computationally-expensive PnP component.
% \julieta{TODO-- not super happy with this... might rewrite later.}

% \paragraph{Uncertainty propagation:}
% \julieta{This is not happening.}

\subsection{Designing an LPnP System}

We now explain our model design choices, highlighting the ways they overcome
the aforementioned challenges and achieve our design goals.
We show an overview of the proposed architecture in Figure~\ref{fig:architecture}.

\paragraph{Deep GILL:}
As our learning-based localizer we use the state-of-the-art
deep ground intensity LiDAR localizer (Deep GILL)~\cite{deep-gill}.
% 
The idea behind ground intensity localization~\cite{levinson-gill} is to align the (sparse) observed LiDAR sweep $\vec{x}$
with a pre-built (dense) map of the LiDAR intensity patterns of the static scene, $\vec{m}$.
Deep GILL learns deep functions that produce spatial embeddings
of both the map $f(\vec{m})$ and LiDAR sweep $g(\tilde{\vec{x}}_{\text{fine}})$ before alignment,
where $\vec{\tilde{x}}_{\text{fine}}$ represents the LiDAR sweep voxelized at
a resolution of 5 centimetres per voxel.
Following existing work~\cite{deep-gill} we parameterize the vehicle pose using
three degrees of freedom (DoF), $x$, $y$, and yaw, represented as $\xi \in
\mathbb{R}^3$.

Given a small set of pre-defined translational and rotational offsets,
we compute the dot product between the transformed sweep and the map embeddings,
and choose the pose candidate $\xi^*$ from a pre-defined set (near the original
pose estimate)
with the highest correlation as the maximum-likelihood estimate of the vehicle
pose:
\begin{align}
  \label{eq:gill-match}
  \xi^* = \argmax_{\xi} %\left(
	 \pi\!\left(g(\tilde{\vec{x}}_{\text{fine}}, \xi) \cdot f(\vec{m})\right) 
  % \right) 
  \triangleq \argmax_\xi \bp(\xi)
\end{align}
where $\pi$ is a function which warps its first argument based on the 3-DoF
offset $\xi$ and $\cdot$ represents the dot product operator. In practice,
this matching is done more efficiently by observing that these
dot products can be computed in parallel with respect to the translational
portion of the pose candidates by using a larger-region $\vec{m}$
and performing cross-correlation rather than separate dot products:
\begin{align}
  \label{eq:gill-match2}
	\left(\pi_{3}\!\left(g(\tilde{\vec{x}}_{\text{fine}}, \xi_3) \star f(\vec{m})\right)\right)[i, j]
	=  \pi\!\left(g(\tilde{\vec{x}}_{\text{fine}}, \xi) \cdot f(\vec{m}) \right)
\end{align}
where $\pi_3$ is a function which rotates its first argument based on the rotational offset $\xi_3$, 
$[i, j]$ indexes the entry corresponding to the translational offset $(x, y) = (\xi_1, \xi_2)$, and
$\star$ represents the cross-correlation operator.

Learning $f$ and $g$ end-to-end
produces representations that are invariant to \lidar{} intensity calibration,
and ignore aspects of the scene irrelevant to localization. Learning
can be performed by treating localization as a classification task and
minimizing the cross-entropy between the discrete distribution of $\bp(\xi)$
and the ground truth pose offset $\bp^{\text{GT}}$ expressed using one-hot
encoding~\cite{deep-gill}:
\begin{equation} \label{eq:gill-loss}
  \mathcal{L}_{\textsc{Loc}} = -\sum_\xi \bp(\xi) \log\bp(\xi)^\text{GT}.
\end{equation}

\paragraph{ILVM:}
For our PnP subsystem, we rely on ILVM~\cite{ilvm}, whose robustness to localization
error we quantified in Section~\ref{sec:effect} -- this corresponds to the lower part
of Figure~\ref{fig:architecture}.
ILVM contains four main submodules. (i) A lightweight network processes a rasterized
semantic map centred at the current vehicle pose. We pass our estimated pose to this module.
(ii) Another neural backbone $h$ extracts features from a coarsely voxelized 
\lidar{} sweep $\vec{\tilde{x}}_{\mathrm{coarse}}$. 
These two features maps are concatenated and passed to (iii) a detector-predictor
that encodes the scene into a latent variable,
and (iv) a graph neural network where each node represents a detected actor,
and samples from the latent variable to create multimodal predictions of the actions for the actors in the scene.

\paragraph{Multi-resolution feature sharing:}
An important advantage of Deep GILL is that in contrast to, \eg, point cloud-based
localizers~\cite{du2020dh3d}, it uses the same BEV input representation as ILVM,
enabling a substantial amount of computation to be shared between both systems.
Nevertheless, while perception-prediction models often use a coarser \lidar{}
voxelization resolution (\eg,
20cm~\cite{fast-and-furious,neural-motion-planner}), matching-based localizers
typically require a finer-grained one to localize robustly~\cite{deep-gill}. 

We bypass this
challenge by upsampling a crop of the \lidar{} feature map computed by the coarse
perception backbone to match the resolution of the finer features in the
localization backbone. We then add the feature maps together using a weighted
sum to produce the final localization embedding, as depicted in
Fig.~\ref{fig:architecture}.
More concretely, the proportion of the perception backbone feature map to
crop is determined by the proportion of the spatial dimensions (measured in
meters) of $\vec{\tilde{x}}_{@.05}$ relative to the spatial dimensions of
$\vec{\tilde{x}}_{@.20}$. After passing the cropped feature map through a
convolution layer with one ouput channel, bilinear upsampling is performed to
obtain an embedding of the same width and height (in pixels) as
$\vec{\tilde{x}}_{@.05}$ so that the weighted sum involves same-sized
embeddings of the spatial region of $\vec{\tilde{x}}_{@.05}$.
%\andreib{John, can you please give a bit more details about how much our
%localization net downsamples vs.\ the perception one?}

This setting allows localization \lidar{} embeddings to be computed with very
little run-time or memory overhead compared to the base perception-prediction network.


\paragraph{Side-tuning:}
% \julieta{explain how this is trained end-to-end,
% with an emphasis on the stability and complexity advantages.}
We optimize the full model using side-tuning~\cite{side-tuning}, with the
perception-prediction branch, which is trained on its own first,
acting as a base network, and the \lidar{} branch
of the localizer acting as the side-tuned module. Note that the map embedding
network does not share any weights or feature maps, as all map embeddings can
be pre-computed offline.

We freeze the weights of the perception-prediction network, and only learn the
map and online branches of the localizer, optimizing the Deep GILL loss from
Eq.~\eqref{eq:gill-loss}, leveraging the PnP feature maps in the process. 
The benefits of this approach are three-fold: first,
there is no risk of catastrophic forgetting in the perception-prediction task,
which can be problematic as it typically requires 3--5$\times{}$ more
computation to train than the localizer alone;
second, we do not need to balance the loss terms of the localization vs.\
perception-prediction, eliminating the need for an additional hyperparameter; 
third, training the localizer network can be done much faster than the full
system, since the PnP header no longer needs to be evaluated and fewer
gradients needs to be stored.

\subsection{Implementation details}
\john{
$f$ and $g$ are given the same architecture,
which is a slightly modified version of the architecture
used by the ILVM rasterized HD map backbone (which is itself 
a smaller version of the ILVM \lidar{} backbone). The modifications
we make are to adjust the padding in the first convolutional layer to accomodate
odd-dimensioned input, and reduce the number of convolutional layers in the header from 5 to 1,
giving a total number of convolutional layers of 11.
}

\julieta{TODO add other details that may have escaped above.}

